Semantical Analysis of the Logic of Bunched Implications

We give a novel approach to proving soundness and completeness for a logic (henceforth: the object-logic) that bypasses truth-in-a-model to work directly with validity. Instead of working with specific worlds in specific models, we reason with eigenworlds (i.e., generic representatives of worlds) in an arbitrary model. This reasoning is captured by a sequent calculus for a meta-logic (in this case, first-order classical logic) expressive enough to capture the semantics of the object-logic. Essentially, one has a calculus of validity for the object-logic. The method proceeds through the perspective of reductive logic (as opposed to the more traditional paradigm of deductive logic), using the space of reductions as a medium for showing the behavioural equivalence of reduction in the sequent calculus for the object-logic and in the validity calculus. Rather than study the technique in general, we illustrate it for the logic of Bunched Implications (BI), thus IPL and MILL (without negation) are also treated. Intuitively, BI is the free combination of intuitionistic propositional logic and multiplicative intuitionistic linear logic, which renders its meta-theory is quite complex. The literature on BI contains many similar, but ultimately different, algebraic structures and satisfaction relations that either capture only fragments of the logic (albeit large ones) or have complex clauses for certain connectives (e.g., Beth's clause for disjunction instead of Kripke's). It is this complexity that motivates us to use BI as a case-study for this approach to semantics.

==> archive.tex <==
\begin{Lemma} \label{lem:resproofs}
   Resolution proofs are sound and complete for BVSs; that is, a BVS admits an \system{MK}-proof if and only if it admits a resolution proof.
\end{Lemma}
\begin{proof}
      Let $S$ be a BVS, $S = \langle \Sigma_{\logic{BI}}, w \satisfies \Gamma : w \satisfies \phi \rangle$. One direction of the claim is immediate: If $S$ admits a validity proof, then $S$ holds in classical logic since, by Lemma \ref{lem:resrules}, all the rules in \system{MJ}+$\rrn{res}+\lrn{res}$ are sound; hence, by Lemma \ref{lem:snc:mk}, $S$ admits an \system{MJ}-proof. It remains to show that if $S$ admits an $\system{MK}$-proof, then it admits a resolution proof. 
    
    By Lemma \ref{lem:decomposition}, we may assume that whenever a clause in $\Sigma_{\logic{BI}}$ is instantiated (i.e., is principal in $\lrn \forall$), then it is immediately followed in the reductive reading of the proof by $\lrn \implies$ with the instantiated formula as principal. We require to argue that the choice of clause can be restricted such that one of the branches becomes an instance of an axiom. 
    
    Suppose that there is a BVS such that every proof of it contains a pair of $\lrn \forall$ and $\lrn \implies$ with one of the branches not being trivial, then one has a sub-derivation of the following form:
 \begin{prooftree}
     \AxiomC{$\Sigma_{\logic{BI}}, \Psi \proves \bar{\Pi}$}
    \AxiomC{$\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \Phi, \bar{\Pi}$}
    \RightLabel{$\lrn \implies$}
\BinaryInfC{$\Sigma_{\logic{BI}}, \Phi \implies  \Psi, \bar{\Sigma} \proves \bar{\Pi}$}
\RightLabel{$\lrn \forall$}
\UnaryInfC{$\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \bar{\Pi}$}
 \end{prooftree}
\noindent By definition, either $\Phi$ is an atom, in which case $\Phi \not \in \bar{\Sigma}$, or $\Psi$ is an atom, in which case $\Psi \not \in \bar{\Pi}$.  By pattern matching on the structure of atoms, the atom can only be principal in an axiom at the end of the proof if the reverse direction of the same clause is used; for example, if $\Phi$ is the atom, then one has the following:
\begin{prooftree}
\AxiomC{$\Sigma_{\logic{BI}}, \Psi, \bar{\Sigma} \proves \bar{\Pi}$}
     \AxiomC{$\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \Psi, \bar{\Pi}$}
     \AxiomC{$\square$}
     \RightLabel{$\ax$}
        \UnaryInfC{$\Sigma_{\logic{BI}}, \Phi, \bar{\Sigma} \proves \Phi, \bar{\Pi}$}
     \RightLabel{$\lrn \implies$}
     \BinaryInfC{$\Sigma_{\logic{BI}}, \Phi \impliedby \Psi, \bar{\Sigma} \proves \Phi, \bar{\Pi}$}
     \RightLabel{$\lrn\forall$}
    \UnaryInfC{$\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \Phi, \bar{\Pi}$}
    \RightLabel{$\lrn \implies$}
\BinaryInfC{$\Sigma_{\logic{BI}}, \Phi \implies  \Psi, \bar{\Sigma} \proves \bar{\Pi}$}
\RightLabel{$\lrn \forall$}
\UnaryInfC{$\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \bar{\Pi}$}
 \end{prooftree}
It cannot be that the atoms in $\Psi$ are principal in the axioms of both of the remaining  branches \todo{why???}. Hence, the occurrence of $\Psi$ may be removed in the sub-proof of one of sequents, leaving a proof of $\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \bar{\Pi}$. By infinite descent, there is a proof of $\Sigma_{\logic{BI}}, \bar{\Sigma} \proves \bar{\Pi}$ such that every pair of $\lrn \forall$ and $\rrn \implies$ in the reductive reading comprise a resolution.
\end{proof}





\begin{scprooftree}{0.9}
\AxiomC{$\square$}
\UnaryInfC{$\Sigma_{\logic{BI}}, \Psi_\lor, w \satisfies \phi \land \psi \proves w \satisfies \phi \land \psi, w \satisfies \phi \lor \psi$}
 \AxiomC{$\mathcal{D}$}
    \AxiomC{$\mathcal{D}'$}
    \BinaryInfC{ $\Sigma_{\logic{BI}}, \Psi_\lor, w \satisfies \phi, w \satisfies \psi \proves w \satisfies \phi \lor \psi$}
    \UnaryInfC{ $\Sigma_{\logic{BI}}, \Psi_\lor, w \satisfies \phi \with w \satisfies \psi \proves w \satisfies \phi \lor \psi$}
\BinaryInfC{$\Sigma_{\logic{BI}}, \Phi_\land , \Psi_\lor, w \satisfies \phi \land \psi \proves w \satisfies \phi \lor \psi$}
\UnaryInfC{$ \Sigma_{\logic{BI}}, \Phi_\land, w \satisfies \phi \land \psi \proves w \satisfies \phi \lor \psi$}
   \UnaryInfC{$\Sigma_{\logic{BI}}, w \satisfies \phi \land \psi \proves w \satisfies \phi \lor \psi$}
\end{scprooftree}
where $\mathcal{D}$ is
\begin{prooftree}
\AxiomC{$\square$}
\UnaryInfC{ $\Sigma_{\logic{BI}}, w \satisfies \phi, w \satisfies \psi \proves w \satisfies \phi, w \satisfies \psi, w \satisfies \phi \lor \psi$}
\UnaryInfC{ $\Sigma_{\logic{BI}}, w \satisfies \phi, w \satisfies \psi \proves w \satisfies \phi \parr w \satisfies \psi, w \satisfies \phi \lor \psi$}
\end{prooftree}
and $\mathcal{D}'$ is
\begin{prooftree}
    \AxiomC{$\square$}
    \UnaryInfC{ $\Sigma_{\logic{BI}}, w \satisfies \phi , w \satisfies \psi, w \satisfies \phi \lor \psi \proves w \satisfies \phi \lor \psi$}
    \end{prooftree}
    
    Instead, do this:

==> old_resolution_proof.tex <==








\begin{Example} \label{ex:landmodelslor}
Consider the assertion $\phi \land \psi \models \phi \lor \psi$. It may be verified by witnessing a proof of the appropriate BSV in the sequent calculus. Such a proof would unpack the conjunction in the context and the disjunction in the extract; for example, let $\Phi_\land  :=  (w \satisfies \phi \land \psi)  \implies  (w\satisfies \phi \with w \satisfies \psi) $ and $\Psi_\lor := (w \satisfies \phi \lor \psi) \impliedby (w\satisfies \phi \parr w \satisfies \psi)$, then one has the following proof:
\begin{minipage}{0.95\linewidth}
    \begin{prooftree}
    \AxiomC{$\square$ }
    \AxiomC{$\square$}
    \UnaryInfC{$\Sigma_{\logic{BI}}, (w \satisfies \phi), (w \satisfies \psi) \proves (w \satisfies \phi), (w \satisfies \psi)$}
    \RightLabel{$\rrn \parr$}
    \UnaryInfC{$\Sigma_{\logic{BI}}, (w \satisfies \phi), (w \satisfies \psi) \proves (w \satisfies \phi) \parr (w \satisfies \psi)$}
        \AxiomC{$\square$}
        \RightLabel{$\lrn \Rightarrow$}
    \BinaryInfC{$\Sigma_{\logic{BI}}, \Psi_\lor, (w \satisfies \phi), (w \satisfies \psi) \proves (w \satisfies \phi \lor \psi)$}
    \RightLabel{$\lrn \forall$}
    \UnaryInfC{$\Sigma_{\logic{BI}}, (w \satisfies \phi), (w \satisfies \psi) \proves (w \satisfies \phi \lor \psi)$}
    \RightLabel{$\lrn \parr$}
    \UnaryInfC{$\Sigma_{\logic{BI}}, (w \satisfies \phi) \with (w \satisfies \psi) \proves (w \satisfies \phi \lor \psi)$}
    \RightLabel{$\lrn \Rightarrow$}
         \BinaryInfC{$\Sigma_{\logic{BI}}, \Phi_\land, (w \satisfies \phi \land \psi) \proves (w \satisfies \phi \lor \psi)$}
         \RightLabel{$\lrn{\forall}$}
       \UnaryInfC{$\Sigma_{\logic{BI}}, (w \satisfies \phi \land \psi) \proves (w \satisfies \phi \lor \psi)$}
    \end{prooftree}
    \end{minipage}\\[1.5ex]
    
\noindent This proof is eager in that it fully decomposes the instantiated clause before doing anything else, reading reductively. In contrast,  the handling of disjunction and conjunction could have been interleaved; for example, after the first $\lrn \forall $ in the reductive reading of the proof, producing $\Phi_\land$ in the context, one could have made a second $\lrn \forall$ reduction, producing $\Psi_\lor$.
\end{Example}



\subsubsection{Principled Proofs} It remains to establish a structure to proofs of BVSs that simulates BI's proof theory. These proofs are composed of phases that simulate the application of a rule in BI's sequent calculus for the corresponding BI-sequent. Since these rules are intended to be in correspondence with the use of clauses of satisfaction and the structural rules, these moves become the identifying action of the phases. In order to perform one of these moves, it may be that one needs to access a formula within the context of a bunch (e.g., when simulating the context rules of BI's sequent calculus), hence it may be necessary to \emph{unpack} the context:

\begin{Definition}[Unpacking]
    An unpacking of a BVS is a \system{MK} derivation comprised of closed resolutions on the assertions in the context of the sequents using $\land$-clause and $*$-clause with the assertion as the head of the clause,
    \[
\langle w \satisfies \Gamma : \Pi \rangle  \rightsquigarrow 
\langle \Sigma_{w \satisfies \Gamma}, \Pi \rangle
\]
\end{Definition}
\begin{Example}
The following is representative computation for unpacking a sequent:
\[
\begin{array}{rcl}
\langle \aunit \fatcomma (w \satisfies \munit \fatsemi \rm p \land \rm  q)  : \Pi \rangle & \rightsquigarrow &
\langle R(w,u,v), (u \satisfies \aunit), (v \satisfies \munit \fatsemi \rm p \land \rm q)   : \Pi \rangle \\
& \rightsquigarrow & \langle R(w,u,v), (u \satisfies \aunit), (v \satisfies \munit), (v \satisfies \rm p \land \rm q)   : \Pi \rangle
\end{array}
\]
\end{Example}

The notation $\Sigma_{w \satisfies \Gamma}$ denotes a theory that arises from an unpacking, such that for BI-frames, the theory $\Sigma_{w \satisfies \Gamma}$ is equivalent to $w \satisfies \Gamma$. 

Unpackings do not have to be total; that is, one can have $w \satisfies \Gamma(\phi)$ unpack to a theory $\Sigma_{w \satisfies \Gamma(\phi)}$ containing a meta-formula $x \satisfies \phi$ such that the $\phi$ in the original meta-atom is the same as the $\phi$ in this meta-atom. In this case, the theory may be denoted $\Sigma_{w \satisfies \Gamma(\phi), x \satisfies\phi}$

\begin{Lemma}[Packing] \label{lem:packing}
    $\Sigma_{\logic{BI}}, \Sigma_{w \satisfies \Gamma(\phi), x \satisfies\phi} \proves \Pi$ iff $\Sigma_{\logic{BI}}, (w \satisfies \Gamma(\phi)) \proves \Pi$.
\end{Lemma}
\begin{proof}
If  $\Sigma_{\logic{BI}}, \Sigma_{w \satisfies \Gamma(\phi), (x \satisfies\phi)} \proves \Pi$, then  $\Sigma_{\logic{BI}}, (w \satisfies \Gamma(\phi)) \proves \Pi$ by using the $\land$-clause and $*$-clause deductively. The other direction holds by cut,
\[
\infer{\Sigma_{\logic{BI}}, \Sigma_{w \satisfies \Gamma(\phi), x \satisfies\phi} \proves \Pi}{ \Sigma_{\logic{BI}}, \Sigma_{w \satisfies \Gamma(\phi), x \satisfies\phi} \proves (w \satisfies \Gamma(\phi)) & \Sigma_{\logic{BI}}, (w \satisfies \Gamma(\phi)) \proves \Pi}
\]
\end{proof}

In order to apply packing, it is essential that the sequent is of the right shape, which may require some auxiliary information in the context may be removed:

\begin{Lemma}[Restriction] \label{lem:restriction}
 If $\Sigma_{\logic{BI}}, \Sigma_{w \satisfies \Gamma} \proves (u \satisfies \phi)$, then for some $\Sigma_{u \satisfies \Delta} \subseteq \Sigma_{w \satisfies \Gamma}$ it is the case that $\Sigma_{\logic{BI}}, \Sigma_{u \satisfies \Delta} \proves (u \satisfies \phi)$.
\end{Lemma}
\begin{proof}
If $u = \pi$, the claim is trivial, similarly if $\phi$ is a validity (i.e., it holds at any world in any model), so assume not. We proceed by induction on the depth of $\Gamma$; that is, on the maximal number of multiplicative context-formers or connectives it contains from root to leaf. 

\textsc{Base Case.} Suppose $\Gamma$ contains only additive context-formers, then $\Sigma_{w \satisfies \Gamma} = (w \satisfies \phi_1),...,(w\satisfies\phi_n)$ with the $\phi_i$ implications or atomic BI-formulas. Hence, since $\Sigma_{\logic{BI}}, \Sigma_w \proves (u \satisfies \phi)$, it must be that $w = u$ because otherwise the extract cannot have interacted with any formula in the context. Since $\Sigma_w = \Sigma_u$, taking $\Sigma_w = \Sigma_u$ established the claim.

\textsc{Induction Step.} Suppose $\Gamma$ contains at least one multiplicative context-former, then $\Sigma_{w \satisfies \Gamma} =  R(w,w_1,w_2) \cup \Sigma_{w_1 \satisfies \Delta_1}\cup\Sigma_{w_2 \satisfies \Delta_2}\cup \Sigma_{w \satisfies \Delta}$ such that $u$ appears in  $\Sigma_{w_1 \satisfies \Delta_1}$ ---  it must appear somewhere for validity to hold, and without loss of generality it appears in this theory. Hence, since $\Sigma_{\logic{BI}}, \Sigma_w \proves (u \satisfies \phi)$, it must be that $\Sigma_{\logic{BI}}, \Sigma_{w_1 \satisfies \Delta_1} \proves (u \satisfies \phi)$ as the other theories cannot not interact with the $u \satisfies \phi$ since the world-variable does not appear in them. By induction hypothesis, there $\Sigma_{u \satisfies \Delta} \subseteq \Sigma_{w_1 \satisfies \Delta_1} \subset \Sigma_{w \satisfies \Gamma}$ such that $\Sigma_{\logic{BI}}, \Sigma_{u \satisfies \Delta} \proves (u \satisfies \phi)$.
\end{proof}

Henceforth, \system{MK} is taken to include restriction, packing, and unpacking, which are admissible by Lemma \ref{lem:restriction} and Lemma \ref{lem:packing}.

The phasal structure of proof can finally be given:

\begin{Definition}[Principled Derivation] \label{def:clausalproof}
    A derivation whose premisses and conclusion are BVSs is principled if it satisfies the following structure in the reductive reading:
    \begin{itemize}
        \item The BVS is unpacked;
        \item Either a resolution is performed, a structural rule is applied, or an axiom rule is applied;
        \item Any non-assertions are either decomposed or resolved in the context and any meta-sequents with non-assertions in the extract are proved;
        \item The resulting sequents are restricted and packed to form BVSs. 
    \end{itemize}
\end{Definition}

    The resolution or the structural rule applied in the second step in the a principled derivation is called the \emph{principal move} of the derivation.

\begin{Definition}[Principled Proof]
    A proof is principled if it is composed of principled derivations. 
\end{Definition}

The proof in Example \ref{ex:instimpl} is principled. It is composed of two principal derivations; the first resolves with the $\land$-clause as the principal move, and the second resolves with $\lor$-clause as the principal move.
 
\begin{Theorem}\label{thm:resproofs}
   If a BVS is provable, then it has a world-conservative, intuitionistic, principled proof.
\end{Theorem}
\begin{proof}
 Let $S$ be a provable BVS; by Lemma \ref{lem:intuitionistic}, it has a world-conservative and intuitionistic proof $\mathcal{D}$. We proceed by induction on the maximal number of moves  in any branch of $\mathcal{D}$ to show that a world-conservative, intuitionistic, principled proof of $S$ exists.

\textsc{Base Case.} Suppose $\mathcal{D}$ only contains one move, then it must be an axiom. A world-conservative, intuitionistic, principled proof of $S$ is given by doing an unpacking to make the axiom  rule applicable and then applying it. 

\todo{do reductions, because now if you make a mistake with a non-invertible rule, who cares? A proof must exist, it is one where you did the perparatory steps first}
\textsc{Induction Step.}
We construct a principled derivation $\mathcal{D}'$ of $S$ with the first move of $\mathcal{D}$ as the principal move. The derivation $\mathcal{D}'$ begins with an unpacking (since it is invertible, by Lemma \ref{lem:packing}) to make the first move of $\mathcal{D}$ applicable and the applies it and decomposed or resolves the resulting non-assertions. It then restricts and packs the resulting sequents producing provable BVS, justified by Lemma \ref{lem:restriction} and Lemma \ref{lem:packing}. These BVSs have proofs with strictly fewer moves than $\mathcal{D}$ since they may be proved with the remaining moves in the proof. Hence, by induction hypothesis, they admit world-conservative, intuitionistic, principled proofs. By composing thse proofs with $\mathcal{D}'$, one has a world-conservative, intuitionistic, principled proof of $S$ too. 
\end{proof}

It is these world-conservative, intuitionistic, and principled that are the resolution proofs simulating BI's sequent calculus:

\begin{Definition}[Resolution Proof]
    A proof of a BVS that is intuitionistic,  world-conservative, and principled is a resolution proof.
\end{Definition}
















